Elemental Abundances and their Implications for the Chemical Enrichment of the Bo\"{o}tes~I Ultra-Faint Galaxy

We present a double-blind analysis of high-dispersion spectra of seven red giant members of the Bo\"{o}tes I ultra-faint dwarf spheroidal galaxy, complemented with re-analysis of a similar spectrum of an eighth member star. The stars cover [Fe/H] from -3.7 to -1.9, and include a CEMP-no star with [Fe/H] = -3.33. We conclude from our chemical abundance data that Bo\"{o}tes I has evolved as a self-enriching star-forming system, from essentially primordial initial abundances. This allows us uniquely to investigate the place of CEMP-no stars in a chemically evolving system, in addition to limiting the timescale of star formation. The elemental abundances are formally consistent with a halo-like distribution, with enhanced mean [alpha/Fe] and small scatter about the mean. This is in accord with the high-mass stellar IMF in this low-stellar-density, low-metallicity system being indistinguishable from the present-day solar neighborhood value. There is a non-significant hint of a decline in [alpha/Fe] with [Fe/H]; together with the low scatter, this requires low star formation rates, allowing time for SNe ejecta to be mixed over the large spatial scales of interest. One star has very high [Ti/Fe], but we do not confirm a previously published high value of [Mg/Fe] for another star. We discuss the existence of CEMP-no stars, and the absence of any stars with lower CEMP-no enhancements at higher [Fe/H], a situation which is consistent with knowledge of CEMP-no stars in the Galactic field. We show that this observation requires there be two enrichment paths at very low metallicities: CEMP-no and "carbon-normal".

==> tab4.tex <==
\begin{deluxetable*}{lccrrrrrrrrrrrrrrr}
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{18}                                                                                                       
\tablewidth{0pt}                                                                                                        
\tablecaption{\label{Tab:nyeweps}NY ATOMIC DATA, EQUIVALENT WIDTHS (m{\AA}), AND ABSOLUTE ABUNDANCES}
\tablehead{
\colhead {Spec.} & {$\lambda$} & {$\chi$} & {\loggf} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$}  & {EW}     & {log\,$\epsilon$} & {EW}     & {log\,$\epsilon$} \\
          {}  &   {(\AA)}      &  {(eV)} &  {}     & {Boo33} & {Boo33}      & {Boo41} &   {Boo41}    & {Boo94} & {Boo94}   & {Boo117} & {Boo117}     & {Boo119} & {Boo119}      & {Boo127} & {Boo127}     & {Boo130} & {Boo130} \\
({1}) & ({2}) & ({3}) & ({4}) & ({5}) & ({6}) & ({7}) & ({8}) & ({9}) & ({10}) & ({11}) & ({12}) & ({13}) & ({14}) & ({15}) & ({16}) & ({17}) & ({18})
}                                                                                                                       
\startdata                                                                                                              
Na\,I    &  5895.92 &   0.00 &  $-$0.19 & 191.0 &  3.90 &   ... &   ... & 164.5 &  3.22 &   ... &   ... & 155.0 &  3.73 &   ... &   ... & 185.0 &  3.92 \\
Mg\,I    &  5528.40 &   4.34 &  $-$0.34 & 108.0 &  5.42 & 168.5 &  6.16 &  81.3 &  4.98 & 104.5 &  5.36 &  90.7 &  5.33 & 127.0 &  5.63 &  99.4 &  5.35 \\
Ca\,I    &  5349.47 &   2.71 &  $-$0.31 &  17.5 &  4.00 &  59.8 &  4.70 &   ... &   ... &  31.0 &  4.28 &   ... &   ... &  39.5 &  4.39 &   ... &   ... \\
Ca\,I    &  5581.98 &   2.52 &  $-$0.71 &   ... &   ... &  46.3 &  4.69 &   ... &   ... &  37.2 &  4.55 &   ... &   ... &  44.9 &  4.64 &   ... &   ... \\
Ca\,I    &  5588.75 &   2.52 &   0.21 &  82.4 &  4.27 & 118.5 &  4.72 &   ... &   ... &  83.6 &  4.27 &  18.0 &  3.32 &  98.5 &  4.43 &  78.2 &  4.25 \\
Ca\,I    &  5590.13 &   2.52 &  $-$0.71 &  25.2 &  4.36 &  58.3 &  4.85 &   ... &   ... &  31.5 &  4.46 &   ... &   ... &  34.8 &  4.48 &   ... &   ... \\
Ca\,I    &  5857.45 &   2.93 &   0.23 &  35.5 &  4.08 &  64.8 &  4.47 &  17.4 &  3.63 &  56.3 &  4.36 &   ... &   ... &  52.7 &  4.28 &  36.0 &  4.10 \\
Ca\,I    &  6102.72 &   1.88 &  $-$0.79 &  46.8 &  4.02 & 104.0 &  4.71 &  38.8 &  3.80 &  60.5 &  4.18 &   ... &   ... &  84.2 &  4.43 &  34.8 &  3.87 \\
Ca\,I    &  6122.22 &   1.89 &  $-$0.32 &  72.8 &  3.90 & 164.0 &  5.09 &  69.4 &  3.73 & 102.5 &  4.26 &  30.2 &  3.37 & 128.5 &  4.57 & 104.0 &  4.36 \\
Ca\,I    &  6162.17 &   1.90 &  $-$0.09 & 104.0 &  4.08 & 146.0 &  4.61 &  76.9 &  3.59 & 127.5 &  4.39 &  61.8 &  3.65 & 147.0 &  4.62 &  87.9 &  3.91 \\
Ca\,I    &  6169.56 &   2.53 &  $-$0.48 &   ... &   ... &  57.0 &  4.59 &  10.4 &  3.61 &  23.7 &  4.06 &   ... &   ... &  37.4 &  4.28 &   ... &   ... \\
Ca\,I    &  6439.08 &   2.52 &   0.47 &   ... &   ... & 136.5 &  4.64 &  55.5 &  3.52 &  84.1 &  3.97 &  26.3 &  3.23 & 116.5 &  4.36 &  73.9 &  3.89 \\
Ca\,I    &  6493.79 &   2.52 &  $-$0.11 &  70.1 &  4.39 & 120.5 &  5.00 &   ... &   ... &  61.3 &  4.26 &   ... &   ... &  80.8 &  4.47 &   ... &   ... \\
Sc\,II   &  5031.02 &   1.36 &  $-$0.40 &  40.0 &  0.53 &   ... &   ... &  44.8 &  0.28 &  61.5 &  0.80 &   ... &   ... &  73.0 &  0.99 &  52.2 &  0.73 \\
Sc\,II   &  5526.79 &   1.77 &   0.03 &  45.5 &  0.64 &   ... &   ... &  38.1 &  0.23 &  63.2 &  0.85 &   ... &   ... &  69.0 &  0.97 &   ... &   ... \\
Sc\,II   &  5657.88 &   1.51 &  $-$0.60 &  32.8 &  0.75 &   ... &   ... &   ... &   ... &  46.3 &  0.93 &   ... &   ... &  48.5 &  1.02 &   ... &   ... \\
Ti\,I    &  4981.73 &   0.84 &   0.50 &  52.5 &  2.16 &   ... &   ... &  55.0 &  2.02 &  85.1 &  2.54 &   ... &   ... &  90.9 &  2.54 &   ... &   ... \\
Ti\,I    &  4991.06 &   0.84 &   0.38 &  53.3 &  2.29 &   ... &   ... &  53.6 &  2.13 &  90.6 &  2.73 &   ... &   ... & 115.0 &  3.01 &   ... &   ... \\
Ti\,I    &  4999.50 &   0.83 &   0.25 &  67.5 &  2.59 &   ... &   ... &  45.2 &  2.14 &  88.9 &  2.82 &   ... &   ... &  87.8 &  2.73 &  55.3 &  2.48 \\
Ti\,I    &  5064.65 &   0.05 &  $-$0.99 &   ... &   ... & 138.5 &  3.79 &  40.2 &  2.34 &  65.8 &  2.81 &   ... &   ... &  89.3 &  3.02 &   ... &   ... \\
Ti\,I    &  5173.75 &   0.00 &  $-$1.12 &  57.3 &  2.81 & 128.5 &  3.68 &  35.7 &  2.33 &   ... &   ... &   ... &   ... & 106.5 &  3.30 &  38.5 &  2.60 \\
Ti\,I    &  5192.97 &   0.02 &  $-$1.01 &   ... &   ... &   ... &   ... &   ... &   ... &  70.8 &  2.84 &   ... &   ... &  95.8 &  3.06 &   ... &   ... \\
Ti\,I    &  5210.38 &   0.05 &  $-$0.88 &  61.3 &  2.68 &   ... &   ... &  46.2 &  2.30 &  72.7 &  2.77 &   ... &   ... & 101.5 &  3.04 &  60.5 &  2.72 \\
Ti\,II   &  4865.61 &   1.12 &  $-$2.81 &   ... &   ... &   ... &   ... &  23.0 &  2.43 &   ... &   ... &   ... &   ... &   ... &   ... &  46.5 &  3.17 \\
Ti\,II   &  5129.15 &   1.89 &  $-$1.30 &   ... &   ... &   ... &   ... &  44.0 &  2.20 &  75.5 &  2.89 &   ... &   ... &  81.1 &  3.02 &   ... &   ... \\
Ti\,II   &  5185.91 &   1.89 &  $-$1.37 &  32.2 &  2.38 & 123.5 &  3.78 &  29.6 &  2.05 &  51.7 &  2.65 &   ... &   ... &  74.1 &  3.00 &  54.0 &  2.73 \\
Ti\,II   &  5226.54 &   1.57 &  $-$1.23 &  93.4 &  2.67 &   ... &   ... &  76.1 &  2.11 &  91.2 &  2.62 &   ... &   ... & 125.0 &  3.16 &   ... &   ... \\
Ti\,II   &  5336.77 &   1.58 &  $-$1.63 &  78.6 &  2.89 & 166.0 &  4.29 &  60.5 &  2.34 &  79.2 &  2.88 &   ... &   ... &  90.9 &  3.08 &  79.3 &  2.93 \\
Cr\,I    &  5206.04 &   0.94 &   0.02 & 110.0 &  2.70 &   ... &   ... &  93.2 &  2.24 & 132.0 &  3.01 &  36.5 &  1.80 & 158.5 &  3.36 & 120.0 &  2.95 \\
Cr\,I    &  5208.42 &   0.94 &   0.16 &   ... &   ... &   ... &   ... & 115.0 &  2.37 &   ... &   ... &  65.0 &  2.09 &   ... &   ... & 191.0 &  3.99 \\
Cr\,I    &  5247.57 &   0.96 &  $-$1.64 &  20.8 &  3.08 &  76.2 &  3.88 &   ... &   ... &  29.0 &  3.22 &   ... &   ... &   ... &   ... &   ... &   ... \\
Cr\,I    &  5296.70 &   0.98 &  $-$1.40 &  35.1 &  3.14 &  82.2 &  3.72 &  11.7 &  2.45 &  38.5 &  3.16 &   ... &   ... &  71.6 &  3.53 &   ... &   ... \\
Cr\,I    &  5345.80 &   1.00 &  $-$0.98 &   ... &   ... & 111.5 &  3.71 &   ... &   ... &  64.0 &  3.11 &   ... &   ... &  87.8 &  3.34 &  68.7 &  3.25 \\
Cr\,I    &  5348.33 &   1.00 &  $-$1.29 &  44.3 &  3.19 & 102.0 &  3.90 &   ... &   ... &  60.8 &  3.38 &   ... &   ... &  79.7 &  3.54 &   ... &   ... \\
Cr\,I    &  5409.77 &   1.03 &  $-$0.72 &  55.5 &  2.81 & 111.0 &  3.47 &  29.5 &  2.28 &  85.0 &  3.14 &   ... &   ... &  98.5 &  3.25 &  61.0 &  2.92 \\
Fe\,I    &  4871.32 &   2.87 &  $-$0.36 &   ... &   ... & 174.0 &  5.86 &  87.6 &  4.37 & 140.5 &  5.38 &   ... &   ... & 163.0 &  5.70 & 118.5 &  5.12 \\
Fe\,I    &  4872.14 &   2.88 &  $-$0.57 &   ... &   ... &   ... &   ... &  60.5 &  4.27 & 112.0 &  5.12 &   ... &   ... & 139.0 &  5.52 &  84.5 &  4.79 \\
Fe\,I    &  4891.49 &   2.85 &  $-$0.11 &   ... &   ... & 135.0 &   ... &  96.0 &  4.19 & 148.5 &  5.24 &  78.2 &  4.32 &   ... &   ... & 129.5 &  5.04 \\
Fe\,I    &  4918.99 &   2.87 &  $-$0.34 & 113.5 &  4.92 & 123.5 &   ... &  77.9 &  4.23 & 122.5 &  5.05 &   ... &   ... & 131.5 &  5.14 & 116.0 &  5.05 \\
Fe\,I    &  4920.50 &   2.83 &   0.07 & 129.0 &  4.72 &   ... &   ... & 112.5 &  4.20 & 157.0 &  5.17 &   ... &   ... & 169.0 &  5.30 & 146.0 &  5.12 \\
Fe\,I    &  4938.81 &   2.87 &  $-$1.08 &  58.5 &  4.88 &   ... &   ... &  44.2 &  4.55 & 120.0 &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
Fe\,I    &  4939.69 &   0.86 &  $-$3.34 & 117.0 &  5.52 & 142.0 &  5.83 &  99.1 &  4.97 & 108.0 &  5.34 &  72.6 &   ... & 131.0 &  5.60 &   ... &   ... \\
Fe\,I    &  4994.13 &   0.92 &  $-$3.08 & 129.5 &  5.52 &   ... &   ... &  90.6 &  4.68 & 134.5 &  5.56 &   ... &   ... & 149.0 &  5.70 &   ... &   ... \\
Fe\,I    &  5001.87 &   3.88 &   0.01 &   ... &   ... &  60.7 &   ... &  23.0 &  4.31 &  54.4 &  4.91 &   ... &   ... &  66.6 &  5.03 &  52.8 &  4.94 \\
Fe\,I    &  5006.12 &   2.83 &  $-$0.62 &  97.2 &  4.89 & 131.5 &  5.37 &  71.4 &  4.38 & 107.0 &  5.01 &   ... &   ... & 129.5 &  5.32 &  99.2 &  4.99 \\
Fe\,I    &  5049.82 &   2.28 &  $-$1.36 & 108.0 &  5.11 & 127.0 &  5.36 &  77.2 &  4.50 & 120.5 &  5.28 &  46.7 &  4.40 & 136.0 &  5.48 &  92.2 &  4.96 \\
Fe\,I    &  5051.63 &   0.92 &  $-$2.80 & 123.0 &  5.12 & 153.5 &  5.53 & 114.5 &  4.69 & 135.5 &  5.28 &  46.7 &  4.23 & 151.0 &  5.44 & 113.5 &  5.08 \\
Fe\,I    &  5068.77 &   2.94 &  $-$1.04 &  67.2 &  5.03 & 109.5 &  5.57 &  26.1 &  4.29 &  59.2 &  4.90 &   ... &   ... &  93.8 &  5.31 &  56.2 &  4.93 \\
Fe\,I    &  5074.75 &   4.22 &  $-$0.20 &  36.2 &  5.26 &  86.9 &  5.94 &   ... &   ... &   ... &   ... &   ... &   ... &  57.0 &  5.51 &  38.2 &  5.32 \\
Fe\,I    &  5079.74 &   0.99 &  $-$3.22 & 101.0 &  5.30 & 119.5 &  5.51 &  72.9 &  4.71 &   ... &   ... &   ... &   ... & 139.5 &  5.75 & 103.0 &  5.41 \\
Fe\,I    &  5083.34 &   0.96 &  $-$2.96 & 132.5 &  5.48 & 152.5 &  5.72 & 100.5 &  4.72 & 124.5 &  5.31 &   ... &   ... & 150.0 &  5.62 & 124.5 &  5.46 \\
Fe\,I    &  5123.72 &   1.01 &  $-$3.07 & 128.0 &  5.57 & 159.0 &  5.99 &  93.8 &  4.81 & 126.0 &  5.50 &   ... &   ... & 141.0 &  5.65 & 126.5 &   ... \\
Fe\,I    &  5127.36 &   0.92 &  $-$3.31 &  90.8 &  5.15 & 112.0 &  5.39 &  82.7 &  4.81 & 100.2 &  5.23 &  26.9 &  4.39 & 118.0 &  5.41 &  95.8 &  5.30 \\
Fe\,I    &  5150.84 &   0.99 &  $-$3.04 & 117.5 &  5.35 & 141.0 &  5.63 &  85.8 &  4.66 & 131.5 &  5.53 &   ... &   ... & 139.0 &  5.54 &  94.2 &  5.09 \\
Fe\,I    &  5151.91 &   1.01 &  $-$3.32 &  72.4 &  5.04 & 125.5 &  5.71 &  69.7 &  4.79 &  99.5 &  5.34 &   ... &   ... & 116.5 &  5.51 &  85.8 &  5.28 \\
Fe\,I    &  5162.27 &   4.18 &   0.02 &  52.2 &  5.23 &  88.7 &  5.69 &   ... &   ... &  54.5 &  5.24 &   ... &   ... &  64.4 &  5.34 &  48.9 &  5.21 \\
Fe\,I    &  5166.28 &   0.00 &  $-$4.20 & 119.0 &  5.31 & 115.0 &  5.16 & 110.0 &  4.84 & 124.0 &  5.32 &  34.2 &  4.31 & 151.0 &  5.61 & 109.0 &  5.25 \\
Fe\,I    &  5171.60 &   1.49 &  $-$1.79 & 145.5 &  5.17 & 149.0 &  5.14 & 118.0 &  4.42 & 139.0 &  5.03 &   ... &   ... & 151.5 &  5.13 & 143.0 &  5.25 \\
Fe\,I    &  5191.46 &   3.04 &  $-$0.55 & 114.5 &  5.31 & 141.0 &  5.67 &  62.1 &  4.44 & 106.0 &  5.15 &   ... &   ... & 129.0 &  5.47 &  95.2 &  5.09 \\
Fe\,I    &  5192.34 &   3.00 &  $-$0.42 &  89.2 &  4.76 & 119.5 &  5.16 &  68.4 &  4.34 & 108.0 &  5.01 &  57.1 &  4.45 & 130.5 &  5.31 &  91.3 &  4.85 \\
Fe\,I    &  5194.94 &   1.56 &  $-$2.09 & 121.0 &  5.15 & 155.0 &  5.62 & 105.0 &  4.64 & 126.5 &  5.20 &   ... &   ... & 142.5 &  5.38 & 110.0 &  5.07 \\
Fe\,I    &  5216.27 &   1.61 &  $-$2.15 & 118.0 &  5.22 & 144.5 &  5.57 &  85.6 &  4.54 & 101.5 &  4.94 &  42.7 &  4.32 & 131.5 &  5.31 & 102.5 &  5.07 \\
Fe\,I    &  5225.53 &   0.11 &  $-$4.79 &  78.2 &  5.47 &  81.9 &  5.46 &  58.5 &  5.00 &  95.7 &  5.64 &   ... &   ... & 101.8 &  5.61 &  62.4 &  5.34 \\
Fe\,I    &  5232.94 &   2.94 &  $-$0.06 & 125.0 &  4.86 & 142.5 &  5.08 &  99.2 &  4.25 & 131.0 &  4.94 &   ... &   ... & 140.5 &  5.03 & 106.5 &   ... \\
Fe\,I    &  5254.96 &   0.11 &  $-$4.76 &  75.2 &  5.40 & 109.0 &  5.76 &   ... &   ... &   ... &   ... &   ... &   ... & 104.5 &  5.61 &   ... &   ... \\
Fe\,I    &  5266.56 &   3.00 &  $-$0.39 &  89.2 &  4.72 & 113.5 &   ... &  63.7 &  4.25 &  89.0 &   ... &   ... &   ... & 119.0 &  5.09 &  94.8 &  4.87 \\
Fe\,I    &  5281.79 &   3.04 &  $-$0.83 &  69.2 &  4.95 & 111.5 &  5.48 &  39.8 &  4.42 &  80.6 &  5.07 &   ... &   ... &  89.8 &  5.15 &  77.6 &  5.11 \\
Fe\,I    &  5283.62 &   3.24 &  $-$0.52 &   ... &   ... &   ... &   ... &  58.2 &  4.60 & 111.5 &  5.44 &   ... &   ... & 135.5 &  5.77 &   ... &   ... \\
Fe\,I    &  5302.31 &   3.28 &  $-$0.88 &   ... &   ... & 108.0 &  5.77 &  26.9 &  4.55 &  69.4 &  5.26 &   ... &   ... &  80.8 &  5.36 &   ... &   ... \\
Fe\,I    &  5307.36 &   1.61 &  $-$2.99 &  57.8 &  5.24 & 103.0 &  5.77 &  31.6 &  4.70 &  67.2 &  5.32 &   ... &   ... &  82.9 &  5.44 &  62.5 &  5.35 \\
Fe\,I    &  5324.18 &   3.21 &  $-$0.24 &  90.6 &  4.84 & 144.0 &  5.59 &  66.1 &  4.38 &  98.9 &  4.93 &   ... &   ... & 122.0 &  5.24 &   ... &   ... \\
Fe\,I    &  5328.04 &   0.92 &  $-$1.47 & 194.0 &  4.88 &   ... &   ... & 194.5 &  4.44 &   ... &   ... & 145.0 &  4.58 &   ... &   ... & 191.5 &  5.00 \\
Fe\,I    &  5328.53 &   1.56 &  $-$1.85 & 140.0 &  5.20 &   ... &   ... & 121.5 &  4.58 & 148.0 &  5.29 &  50.5 &  4.07 &   ... &   ... & 139.0 &  5.30 \\
Fe\,I    &  5339.93 &   3.27 &  $-$0.72 &  88.2 &  5.36 &   ... &   ... &  40.2 &  4.60 &  78.0 &  5.20 &   ... &   ... &  98.3 &  5.43 &  73.9 &  5.22 \\
Fe\,I    &  5369.97 &   4.37 &   0.54 &  61.9 &  5.05 &  95.2 &  5.47 &  17.8 &  4.22 &  69.4 &  5.14 &   ... &   ... &  81.5 &  5.27 &  54.7 &  4.98 \\
Fe\,I    &  5371.49 &   0.96 &  $-$1.65 & 169.5 &  4.72 &   ... &   ... & 165.0 &  4.23 & 181.5 &  4.86 &  97.3 &  3.87 & 197.0 &  4.95 & 158.0 &  4.68 \\
Fe\,I    &  5383.38 &   4.31 &   0.64 &  64.5 &  4.92 & 108.0 &  5.48 &   ... &   ... &  64.1 &  4.89 &   ... &   ... &  91.2 &  5.23 &  63.6 &  4.94 \\
Fe\,I    &  5393.18 &   3.24 &  $-$0.91 &  69.0 &  5.26 &  93.6 &  5.55 &  35.8 &  4.68 &  67.2 &  5.21 &   ... &   ... &  83.4 &  5.37 &  59.8 &  5.18 \\
Fe\,I    &  5397.13 &   0.92 &  $-$1.99 & 168.5 &  4.99 &   ... &   ... & 167.0 &  4.54 & 167.0 &  4.92 & 118.5 &  4.56 & 174.0 &   ... & 173.0 &  5.21 \\
Fe\,I    &  5405.77 &   0.99 &  $-$1.84 & 164.0 &  4.85 & 179.5 &   ... & 156.0 &  4.31 & 162.0 &  4.78 &  94.2 &  4.03 & 183.5 &  4.97 & 161.5 &  4.95 \\
Fe\,I    &  5429.70 &   0.96 &  $-$1.88 & 186.0 &  5.20 &   ... &   ... & 171.5 &  4.54 & 194.0 &  5.26 & 109.0 &  4.30 &   ... &   ... & 166.5 &  5.04 \\
Fe\,I    &  5434.52 &   1.01 &  $-$2.12 & 159.5 &  5.08 & 182.0 &  5.31 & 146.5 &  4.48 & 157.0 &  4.99 &  84.2 &  4.17 & 168.0 &  5.04 & 170.0 &  5.39 \\
Fe\,I    &  5446.92 &   0.99 &  $-$1.91 & 178.0 &  5.14 &   ... &   ... & 169.0 &  4.57 & 194.0 &  5.33 & 103.2 &  4.26 &   ... &   ... & 168.5 &  5.13 \\
Fe\,I    &  5455.61 &   1.01 &  $-$2.09 & 189.0 &  5.51 &   ... &   ... & 156.5 &  4.58 &   ... &   ... &  97.0 &  4.35 &   ... &   ... & 186.0 &  5.61 \\
Fe\,I    &  5497.52 &   1.01 &  $-$2.85 & 128.5 &  5.29 & 150.5 &  5.55 & 103.5 &  4.65 & 128.5 &  5.25 &  39.8 &  4.24 & 145.5 &  5.40 & 123.5 &  5.32 \\
Fe\,I    &  5501.46 &   0.96 &  $-$3.05 & 111.0 &  5.17 & 142.5 &  5.56 &  98.2 &  4.73 & 113.0 &  5.16 &  39.8 &  4.38 & 138.5 &  5.43 & 102.5 &  5.14 \\
Fe\,I    &  5506.78 &   0.99 &  $-$2.80 & 121.5 &  5.12 & 132.5 &  5.20 & 107.5 &  4.62 & 113.5 &  4.96 &   ... &   ... & 138.5 &  5.22 & 127.0 &  5.31 \\
Fe\,I    &  5569.62 &   3.42 &  $-$0.54 &  60.9 &  4.99 &   ... &   ... &  37.0 &  4.54 &  65.1 &  5.02 &   ... &   ... &  87.1 &  5.25 &   ... &   ... \\
Fe\,I    &  5572.84 &   3.40 &  $-$0.31 &   ... &   ... & 136.0 &  5.73 &  57.5 &  4.56 &  93.2 &  5.13 &   ... &   ... & 116.0 &  5.41 &  92.2 &  5.20 \\
Fe\,I    &  5586.76 &   3.37 &  $-$0.14 &  89.0 &  4.89 & 125.5 &  5.37 &  54.3 &  4.31 &  96.1 &  4.97 &   ... &   ... & 120.5 &  5.27 &  79.8 &  4.82 \\
Fe\,I    &  5615.64 &   3.33 &  $-$0.14 & 115.5 &  5.22 & 130.0 &  5.39 &  65.3 &  4.39 & 112.5 &  5.15 &   ... &   ... & 115.0 &  5.14 &   ... &   ... \\
Fe\,I    &  6136.62 &   2.45 &  $-$1.40 &  94.5 &  5.07 &   ... &   ... &  69.0 &  4.57 & 114.0 &  5.30 &   ... &   ... & 124.0 &  5.38 &   ... &   ... \\
Fe\,I    &  6137.69 &   2.59 &  $-$1.40 &  87.6 &  5.15 & 121.5 &  5.56 &  52.0 &  4.55 & 115.0 &  5.49 &   ... &   ... & 123.0 &  5.54 &  92.6 &  5.28 \\
Fe\,I    &  6191.56 &   2.43 &  $-$1.42 & 106.5 &  5.22 & 139.0 &  5.62 &  64.2 &  4.51 & 115.0 &  5.31 &   ... &   ... & 129.0 &  5.44 & 105.0 &  5.27 \\
Fe\,I    &  6213.44 &   2.22 &  $-$2.48 &  43.0 &  5.21 &  75.2 &  5.59 &  17.6 &  4.58 &  53.2 &  5.31 &   ... &   ... &   ... &   ... &  50.7 &  5.36 \\
Fe\,I    &  6219.29 &   2.20 &  $-$2.43 &  54.0 &  5.28 &  80.8 &  5.58 &  25.3 &  4.69 &  67.3 &  5.42 &   ... &   ... &  92.8 &  5.66 &  49.0 &  5.26 \\
Fe\,I    &  6230.72 &   2.56 &  $-$1.28 &  98.7 &  5.13 & 137.0 &  5.61 &  66.4 &  4.55 & 100.0 &  5.12 &   ... &   ... &  99.8 &  5.05 &  89.3 &  5.07 \\
Fe\,I    &  6252.56 &   2.40 &  $-$1.69 &  94.2 &  5.28 & 115.5 &  5.52 &  61.1 &  4.70 & 102.5 &  5.36 &   ... &   ... & 123.0 &  5.58 & 101.9 &  5.46 \\
Fe\,I    &  6393.60 &   2.43 &  $-$1.58 & 103.0 &  5.32 & 123.0 &  5.54 &  56.3 &  4.57 & 106.0 &  5.33 &   ... &   ... & 135.0 &  5.66 &   ... &   ... \\
Fe\,I    &  6400.01 &   3.60 &  $-$0.52 &  56.0 &  5.08 &   ... &   ... &  30.5 &  4.58 &  63.8 &  5.15 &   ... &   ... &  93.8 &  5.49 &  51.5 &  5.05 \\
Fe\,I    &  6421.35 &   2.28 &  $-$2.03 &  67.9 &  5.14 & 102.8 &  5.53 &  42.2 &  4.65 &  84.0 &  5.30 &   ... &   ... & 102.0 &  5.47 &  72.1 &  5.24 \\
Fe\,I    &  6430.85 &   2.18 &  $-$2.01 &  92.7 &  5.30 & 106.5 &  5.44 &  57.7 &  4.70 & 102.2 &  5.39 &   ... &   ... & 118.0 &  5.53 &  94.4 &  5.39 \\
Fe\,I    &  6494.98 &   2.40 &  $-$1.27 &  96.3 &  4.87 & 129.0 &  5.26 &  70.5 &  4.37 & 117.5 &  5.12 &   ... &   ... & 130.0 &  5.23 & 111.5 &  5.15 \\
Fe\,II   &  4923.93 &   2.89 &  $-$1.21 & 132.5 &  4.82 & 160.0 &  5.42 & 120.5 &  4.21 & 133.5 &  4.84 &  44.3 &  3.51 & 154.0 &  5.27 & 142.0 &  5.08 \\
Fe\,II   &  5197.58 &   3.23 &  $-$2.23 &  53.0 &  5.06 & 119.0 &  6.13 &  40.8 &  4.63 &   ... &   ... &   ... &   ... &  83.2 &  5.52 &  64.5 &  5.24 \\
Fe\,II   &  5234.62 &   3.22 &  $-$2.15 &  66.0 &  5.14 &   ... &   ... &   ... &   ... &  74.0 &  5.23 &   ... &   ... &  84.9 &  5.45 &   ... &   ... \\
Fe\,II   &  5325.55 &   3.22 &  $-$3.22 &  19.3 &  5.43 &  32.2 &  5.85 &   ... &   ... &  26.6 &  5.59 &   ... &   ... &   ... &   ... &   ... &   ... \\
Ni\,I    &  5137.07 &   1.68 &  $-$1.99 &  44.0 &  3.87 &   ... &   ... &  32.0 &  3.52 &  70.4 &  4.18 &   ... &   ... &  77.1 &  4.20 &  52.5 &  4.03 \\
Ni\,I    &  5476.90 &   1.83 &  $-$0.89 &  94.0 &  3.57 &   ... &   ... &  80.6 &  3.19 & 110.5 &  3.77 &   ... &   ... & 133.5 &  4.05 & 111.0 &  3.90 \\
Ni\,I    &  6643.64 &   1.68 &  $-$2.01 &  39.0 &  3.72 &  57.0 &  3.94 &  14.3 &  3.03 &  41.0 &  3.71 &   ... &   ... &   ... &   ... &  30.8 &  3.62 \\
Zn\,I    &  4810.53 &   4.08 &  $-$0.14 &   ... &   ... &  56.2 &  2.75 &   ... &   ... &  47.2 &  2.53 &   ... &   ... &   ... &   ... &  40.9 &  2.47 \\
Ba\,II   &  4934.08 &   0.00 &  $-$0.15 & 153.0 & $-$0.43 & 175.0 &  0.07 & 102.8 & $-$1.74 & 168.0 & $-$0.20 &  44.2 & $-$2.03 & 192.0 &  0.23 & 151.5 & $-$0.31 \\
Ba\,II   &  5853.69 &   0.60 &  $-$0.91 &  40.0 & $-$0.68 &  66.1 & $-$0.18 &   ... &   ... &  20.5 & $-$1.08 &   ... &   ... &  36.4 & $-$0.72 &   ... &   ... \\
Ba\,II   &  6141.73 &   0.70 &  $-$0.08 &  95.8 & $-$0.71 & 115.0 & $-$0.29 &  54.3 & $-$1.58 & 102.5 & $-$0.64 &   ... &   ... & 102.0 & $-$0.59 &  73.6 & $-$0.93 \\
Ba\,II   &  6496.91 &   0.60 &  $-$0.38 &  69.4 & $-$0.88 &  98.0 & $-$0.37 &  19.7 & $-$1.98 &  51.1 & $-$1.13 &   ... &   ... &  66.2 & $-$0.89 &  56.7 & $-$0.99 \\
\enddata                                                                                                                
\end{deluxetable*}                                         


==> tab5.tex <==
\begin{deluxetable}{lccrrrrrrrrrrrrrrr}
\tabletypesize{\tiny}                                                                                                   
\tablecolumns{18}                                                                                                       
\tablewidth{0pt}                                                                                                        
\tablecaption{\label{Tab:gmeweps}GM ATOMIC DATA, EQUIVALENT WIDTHS (m{\AA}), AND ABSOLUTE ABUNDANCES}
\tablehead{
\colhead {Spec.} & {$\lambda$} & {$\chi$} & {\loggf} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$} & {EW} & {log\,$\epsilon$}  & {EW}     & {log\,$\epsilon$} & {EW}     & {log\,$\epsilon$}\\
          {}     &   {(\AA)}   &  {(eV)}  &     {} & {Boo33} & {Boo33}      & {Boo41} &   {Boo41}    & {Boo94} & {Boo94}   & {Boo117} & {Boo117}     & {Boo119} & {Boo119}      & {Boo127} & {Boo127}     & {Boo130} & {Boo130}\\
({1}) & ({2}) & ({3}) & ({4}) & ({5}) & ({6}) & ({7}) & ({8}) & ({9}) & ({10}) & ({11}) & ({12}) & ({13}) & ({14}) & ({15}) & ({16}) & ({17}) & ({18})
}                                                                                                                       
\startdata                                                                                                              
%            atomic                      |      33       |      41       |      94       |        117    |     119       |      127      |        130    |

   Na\,I &  5895.924 &   0.000 &  $-$0.184 & 177.6 &  4.04 &   ... &   ... & 154.6 &  3.68 & 177.2 &  4.14 & 167.8 &  3.55 &   ... &   ... &   ... &   ... \\
   Mg\,I &  5528.405 &   4.346 &  $-$0.620 &  93.1 &  5.66 &   ... &   ... &  75.4 &  5.36 & 101.9 &  5.85 &  74.6 &  5.30 & 113.5 &  5.92 &  91.0 &  5.64 \\
   Mg\,I &  5711.088 &   4.346 &  $-$1.833 &   ... &   ... &  49.5 &  6.27 &  10.2 &  5.28 &   ... &   ... &   ... &   ... &  28.4 &  5.84 &   ... &   ... \\
   Si\,I &  5948.541 &   5.082 &  $-$0.780 &   ... &   ... &  26.0 &  5.58 &   ... &   ... &  25.8 &  5.56 &   ... &   ... &  35.4 &  5.72 &   ... &   ... \\
   Ca\,I &  5261.704 &   2.521 &  $-$0.579 &  27.8 &  4.34 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  45.5 &  4.62 &   ... &   ... \\
   Ca\,I &  5265.556 &   2.523 &  $-$0.113 &  53.7 &  4.33 &   ... &   ... &   ... &   ... &  74.9 &  4.75 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ca\,I &  5581.965 &   2.523 &  $-$0.555 &  19.4 &  4.11 &  50.8 &  4.75 &   ... &   ... &  30.8 &  4.38 &   ... &   ... &  46.2 &  4.60 &   ... &   ... \\
   Ca\,I &  5588.749 &   2.526 &   0.358 &  69.2 &  4.10 &   ... &   ... &  55.3 &  3.81 &  69.5 &  4.16 &   ... &   ... &  90.9 &  4.43 &  72.5 &  4.18 \\
   Ca\,I &  5590.114 &   2.521 &  $-$0.571 &   ... &   ... &  43.4 &  4.64 &   ... &   ... &  32.8 &  4.43 &   ... &   ... &  32.1 &  4.36 &   ... &   ... \\
   Ca\,I &  5594.462 &   2.523 &   0.097 &   ... &   ... &   ... &   ... &  26.5 &  3.54 &  72.3 &  4.47 &   ... &   ... &  91.7 &  4.70 &  61.3 &  4.26 \\
   Ca\,I &  5598.480 &   2.521 &  $-$0.087 &  45.8 &  4.16 &   ... &   ... &  22.6 &  3.63 &  70.2 &  4.61 &   ... &   ... &   ... &   ... &  66.3 &  4.52 \\
   Ca\,I &  5601.277 &   2.526 &  $-$0.523 &  38.2 &  4.47 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  50.7 &  4.64 &  39.7 &  4.53 \\
   Ca\,I &  5857.451 &   2.933 &   0.240 &  42.1 &  4.24 &   ... &   ... &  18.6 &  3.68 &  66.1 &  4.67 &   ... &   ... &  65.3 &  4.57 &  38.1 &  4.20 \\
   Ca\,I &  6102.723 &   1.879 &  $-$0.793 &  53.9 &  4.21 &   ... &   ... &  34.7 &  3.79 &  67.2 &  4.45 &   ... &   ... &  86.0 &  4.65 &  55.1 &  4.27 \\
   Ca\,I &  6122.217 &   1.886 &  $-$0.316 &  69.3 &  3.97 &   ... &   ... &  64.3 &  3.81 &   ... &   ... &   ... &   ... &   ... &   ... &  95.9 &  4.42 \\
   Ca\,I &  6162.173 &   1.899 &  $-$0.090 &  96.9 &  4.21 &   ... &   ... &  73.4 &  3.74 &   ... &   ... &  61.9 &  3.57 &   ... &   ... &   ... &   ... \\
   Ca\,I &  6166.439 &   2.521 &  $-$1.142 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  21.1 &  4.67 &  15.0 &  4.57 \\
   Ca\,I &  6169.563 &   2.526 &  $-$0.478 &   ... &   ... &  61.0 &  4.80 &   ... &   ... &  31.7 &  4.30 &   ... &   ... &   ... &   ... &  25.6 &  4.20 \\
   Ca\,I &  6439.075 &   2.526 &   0.390 &  82.3 &  4.24 &   ... &   ... &  51.9 &  3.67 &  86.3 &  4.38 &   ... &   ... &   ... &   ... &  82.5 &  4.26 \\
   Ca\,I &  6449.808 &   2.521 &  $-$0.502 &  17.5 &  3.96 &  64.1 &  4.86 &  17.4 &  3.87 &  29.9 &  4.27 &   ... &   ... &  41.9 &  4.43 &   ... &   ... \\
   Ca\,I &  6471.662 &   2.526 &  $-$0.686 &  18.9 &  4.19 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  30.6 &  4.41 &   ... &   ... \\
   Ca\,I &  6493.781 &   2.521 &  $-$0.109 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  74.9 &  4.63 \\
   Ca\,I &  6499.650 &   2.523 &  $-$0.818 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  23.1 &  4.38 &   ... &   ... \\
   Ca\,I &  6717.681 &   2.709 &  $-$0.524 &   ... &   ... &   ... &   ... &  14.2 &  4.00 &   ... &   ... &   ... &   ... &  27.4 &  4.39 &   ... &   ... \\
  Sc\,II &  5031.021 &   1.357 &  $-$0.400 &  40.3 &  0.62 &  58.1 &  0.90 &  44.9 &  0.37 &  66.5 &  1.09 &   ... &   ... &  90.4 &  1.43 &  50.5 &  0.79 \\
  Sc\,II &  5239.813 &   1.455 &  $-$0.765 &   ... &   ... &  26.6 &  0.84 &  18.4 &  0.31 &  39.2 &  1.09 &   ... &   ... &  46.0 &  1.17 &  25.1 &  0.81 \\
  Sc\,II &  5526.790 &   1.768 &   0.024 &  41.5 &  0.67 &   ... &   ... &  45.0 &  0.42 &  59.4 &  0.99 &   ... &   ... &  72.8 &  1.15 &  60.1 &  0.95 \\
  Sc\,II &  5641.001 &   1.500 &  $-$1.131 &   ... &   ... &   ... &   ... &  12.5 &  0.50 &  21.9 &  1.13 &   ... &   ... &   ... &   ... &   ... &   ... \\
  Sc\,II &  5657.896 &   1.507 &  $-$0.603 &  37.3 &  0.91 &  49.2 &  1.10 &   ... &   ... &  48.6 &  1.12 &   ... &   ... &  55.7 &  1.19 &  41.5 &  0.98 \\
  Sc\,II &  5669.042 &   1.500 &  $-$1.200 &   ... &   ... &  28.8 &  1.35 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
  Sc\,II &  5684.202 &   1.507 &  $-$1.074 &   ... &   ... &   ... &   ... &  10.6 &  0.37 &   ... &   ... &   ... &   ... &   ... &   ... &  16.9 &  0.94 \\
  Sc\,II &  6604.601 &   1.357 &  $-$1.309 &   ... &   ... &  33.5 &  1.32 &   ... &   ... &   ... &   ... &   ... &   ... &  39.0 &  1.39 &   ... &   ... \\
   Ti\,I &  4840.874 &   0.900 &  $-$0.509 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  4981.731 &   0.848 &   0.504 &  70.9 &  2.58 &   ... &   ... &  56.3 &  2.20 &   ... &   ... &   ... &   ... &   ... &   ... &  62.1 &  2.50 \\
   Ti\,I &  4991.065 &   0.836 &   0.380 &  57.2 &  2.47 &   ... &   ... &  53.0 &  2.25 &  96.5 &  3.28 &   ... &   ... &   ... &   ... &  64.6 &  2.65 \\
   Ti\,I &  4997.096 &   0.000 &  $-$2.118 &   ... &   ... &  46.0 &  3.86 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  4999.503 &   0.826 &   0.250 &  58.0 &  2.60 &   ... &   ... &  58.6 &  2.46 &   ... &   ... &   ... &   ... &  94.2 &  3.15 &  55.4 &  2.62 \\
   Ti\,I &  5007.210 &   0.818 &   0.112 &   ... &   ... &   ... &   ... &  45.3 &  2.37 &   ... &   ... &  26.6 &  2.19 &   ... &   ... &   ... &   ... \\
   Ti\,I &  5016.161 &   0.848 &  $-$0.574 &   ... &   ... &   ... &   ... &   ... &   ... &  51.9 &  3.39 &   ... &   ... &  65.7 &  3.49 &   ... &   ... \\
   Ti\,I &  5020.026 &   0.836 &  $-$0.414 &   ... &   ... &   ... &   ... &  24.0 &  2.51 &  28.2 &  2.78 &   ... &   ... &  71.5 &  3.41 &  43.3 &  3.11 \\
   Ti\,I &  5022.868 &   0.826 &  $-$0.434 &   ... &   ... &  84.1 &  3.76 &  18.8 &  2.38 &   ... &   ... &   ... &   ... &  54.1 &  3.14 &   ... &   ... \\
   Ti\,I &  5024.844 &   0.818 &  $-$0.602 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  29.3 &  2.88 &   ... &   ... \\
   Ti\,I &  5035.903 &   1.460 &   0.243 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  47.0 &  3.12 &   ... &   ... \\
   Ti\,I &  5036.464 &   1.443 &   0.130 &   ... &   ... &   ... &   ... &   ... &   ... &  29.3 &  2.98 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  5038.397 &   1.430 &   0.013 &   ... &   ... &   ... &   ... &   ... &   ... &  30.2 &  3.10 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  5039.957 &   0.021 &  $-$1.130 &   ... &   ... &   ... &   ... &   ... &   ... &  53.9 &  2.97 &   ... &   ... &  94.9 &  3.54 &   ... &   ... \\
   Ti\,I &  5064.653 &   0.048 &  $-$0.991 &   ... &   ... &  97.8 &  3.63 &  32.1 &  2.27 &  53.3 &  2.86 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  5147.478 &   0.000 &  $-$2.012 &   ... &   ... &  60.5 &  3.96 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  5173.743 &   0.000 &  $-$1.118 &   ... &   ... &   ... &   ... &  36.0 &  2.41 &  72.4 &  3.24 &   ... &   ... &  99.6 &  3.57 &  44.0 &  2.81 \\
   Ti\,I &  5192.969 &   0.021 &  $-$1.006 &  27.9 &  2.36 &   ... &   ... &  34.2 &  2.28 &  56.5 &  2.88 &   ... &   ... &  84.1 &  3.19 &  49.5 &  2.81 \\
   Ti\,I &  5210.385 &   0.048 &  $-$0.884 &  56.5 &  2.75 &   ... &   ... &  47.3 &  2.42 &   ... &   ... &   ... &   ... &  89.9 &  3.20 &  70.6 &  3.04 \\
   Ti\,I &  5866.451 &   1.067 &  $-$0.840 &   ... &   ... &  52.2 &  3.88 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ti\,I &  6258.706 &   1.460 &  $-$0.240 &   ... &   ... &  48.5 &  3.67 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
  Ti\,II &  4865.611 &   1.116 &  $-$2.790 &   ... &   ... &  91.2 &  3.95 &   ... &   ... &  38.4 &  3.11 &   ... &   ... &  65.5 &  3.52 &   ... &   ... \\
  Ti\,II &  5129.152 &   1.892 &  $-$1.240 &  68.8 &  2.94 &   ... &   ... &  43.2 &  2.23 &  79.4 &  3.19 &   ... &   ... &  89.8 &  3.30 &  67.8 &  2.91 \\
  Ti\,II &  5154.068 &   1.566 &  $-$1.750 &  59.0 &  2.90 &   ... &   ... &  39.8 &  2.28 &  69.1 &  3.12 &  39.0 &  2.43 &  79.4 &  3.22 &  62.8 &  2.95 \\
  Ti\,II &  5185.902 &   1.893 &  $-$1.490 &  30.1 &  2.54 &   ... &   ... &  34.3 &  2.32 &  58.5 &  3.06 &   ... &   ... &  65.5 &  3.13 &  49.4 &  2.87 \\
  Ti\,II &  5336.771 &   1.582 &  $-$1.590 &   ... &   ... &   ... &   ... &  52.9 &  2.34 &  73.1 &  3.03 &   ... &   ... &  78.0 &  3.04 &  63.3 &  2.80 \\
  Ti\,II &  5381.015 &   1.566 &  $-$1.920 &  36.2 &  2.68 & 102.5 &  3.75 &  33.5 &  2.31 &   ... &   ... &   ... &   ... &  75.1 &  3.30 &  52.8 &  2.95 \\
  Ti\,II &  5418.751 &   1.582 &  $-$2.000 &  26.2 &  2.59 & 103.6 &  3.86 &  26.9 &  2.28 &  52.9 &  3.08 &   ... &   ... &  55.2 &  3.08 &  39.3 &  2.84 \\
   Cr\,I &  5208.425 &   0.941 &   0.158 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  84.8 &  2.26 &   ... &   ... &   ... &   ... \\
   Cr\,I &  5247.565 &   0.961 &  $-$1.640 &   ... &   ... &  81.7 &  4.25 &   ... &   ... &   ... &   ... &   ... &   ... &  48.1 &  3.58 &   ... &   ... \\
   Cr\,I &  5296.691 &   0.983 &  $-$1.400 &  37.1 &  3.25 &   ... &   ... &   ... &   ... &  36.5 &  3.26 &   ... &   ... &  72.0 &  3.74 &   ... &   ... \\
   Cr\,I &  5298.272 &   0.983 &  $-$1.150 &  48.9 &  3.20 &   ... &   ... &  14.2 &  2.30 &  61.4 &  3.44 &   ... &   ... &  67.8 &  3.42 &  60.8 &  3.44 \\
   Cr\,I &  5300.745 &   0.983 &  $-$2.120 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  19.2 &  3.66 \\
   Cr\,I &  5345.796 &   1.004 &  $-$0.980 &  49.0 &  3.05 & 111.7 &  4.18 &  27.4 &  2.51 &  70.8 &  3.46 &   ... &   ... &  93.5 &  3.72 &  71.0 &  3.45 \\
   Cr\,I &  5348.315 &   1.004 &  $-$1.290 &  33.5 &  3.10 & 100.4 &  4.27 &  12.8 &  2.42 &  48.3 &  3.38 &   ... &   ... &  87.6 &  3.92 &  59.9 &  3.59 \\
   Cr\,I &  5409.784 &   1.030 &  $-$0.720 &  63.5 &  3.05 &   ... &   ... &  32.0 &  2.37 &  93.5 &  3.68 &   ... &   ... & 100.3 &  3.61 &  77.5 &  3.32 \\
   Fe\,I &  4859.741 &   2.875 &  $-$0.764 &  66.2 &  4.84 &   ... &   ... &  54.1 &  4.52 &  91.4 &  5.41 &   ... &   ... &   ... &   ... &  85.5 &  5.21 \\
   Fe\,I &  4871.317 &   2.865 &  $-$0.363 &  94.4 &  4.95 &   ... &   ... &  70.8 &  4.41 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  4872.136 &   2.882 &  $-$0.567 &   ... &   ... &   ... &   ... &  58.9 &  4.42 &   ... &   ... &  25.9 &  3.93 &   ... &   ... &   ... &   ... \\
   Fe\,I &  4890.754 &   2.875 &  $-$0.394 &   ... &   ... &   ... &   ... &  68.9 &  4.42 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  4891.492 &   2.851 &  $-$0.112 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  76.2 &  4.16 &   ... &   ... &   ... &   ... \\
   Fe\,I &  4903.308 &   2.882 &  $-$0.926 &  63.9 &  4.97 &   ... &   ... &   ... &   ... &  80.2 &  5.34 &   ... &   ... &  99.4 &  5.55 &   ... &   ... \\
   Fe\,I &  4918.993 &   2.865 &  $-$0.342 &   ... &   ... &   ... &   ... &  84.5 &  4.66 &   ... &   ... &  60.1 &  4.20 &   ... &   ... &   ... &   ... \\
   Fe\,I &  4920.502 &   2.832 &   0.068 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  77.1 &  3.97 &   ... &   ... &   ... &   ... \\
   Fe\,I &  4924.770 &   2.279 &  $-$2.241 &   ... &   ... &   ... &   ... &  30.0 &  4.82 &  85.1 &  6.04 &   ... &   ... &  78.3 &  5.74 &   ... &   ... \\
   Fe\,I &  4938.813 &   2.875 &  $-$1.077 &  46.2 &  4.82 &   ... &   ... &  33.0 &  4.45 &  89.0 &  5.66 &   ... &   ... &  73.8 &  5.21 &   ... &   ... \\
   Fe\,I &  4957.596 &   2.808 &   0.233 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  86.5 &  3.89 &   ... &   ... &   ... &   ... \\
   Fe\,I &  4966.089 &   3.332 &  $-$0.871 &  51.2 &  5.23 &   ... &   ... &  39.4 &  4.92 &  70.6 &  5.62 &   ... &   ... &  80.5 &  5.68 &  67.8 &  5.54 \\
   Fe\,I &  4969.916 &   4.217 &  $-$0.710 &   ... &   ... &   ... &   ... &   ... &   ... &  24.2 &  5.61 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  4973.101 &   3.960 &  $-$0.950 &   ... &   ... &   ... &   ... &   ... &   ... &  42.5 &  5.93 &   ... &   ... &  46.9 &  5.93 &   ... &   ... \\
   Fe\,I &  5001.862 &   3.881 &   0.010 &   ... &   ... &   ... &   ... &  24.7 &  4.40 &   ... &   ... &   ... &   ... &  97.0 &  5.77 &   ... &   ... \\
   Fe\,I &  5002.789 &   3.396 &  $-$1.580 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  41.0 &  5.79 &   ... &   ... \\
   Fe\,I &  5006.117 &   2.832 &  $-$0.638 &   ... &   ... &   ... &   ... &  75.1 &  4.71 &   ... &   ... &  53.1 &  4.36 &   ... &   ... &  99.7 &  5.28 \\
   Fe\,I &  5012.067 &   0.859 &  $-$2.642 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  74.6 &  4.29 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5014.941 &   3.943 &  $-$0.303 &  37.3 &  5.14 &   ... &   ... &   ... &   ... &  52.9 &  5.44 &   ... &   ... &  56.3 &  5.42 &   ... &   ... \\
   Fe\,I &  5022.235 &   3.984 &  $-$0.530 &  24.2 &  5.15 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5028.126 &   3.573 &  $-$1.123 &   ... &   ... &  32.2 &  5.48 &   ... &   ... &   ... &   ... &   ... &   ... &  49.7 &  5.69 &   ... &   ... \\
   Fe\,I &  5044.210 &   2.851 &  $-$2.038 &  28.4 &  5.42 &  74.3 &  6.24 &   ... &   ... &  40.9 &  5.67 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5049.819 &   2.279 &  $-$1.355 &   ... &   ... &   ... &   ... &  71.5 &  4.67 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5051.634 &   0.915 &  $-$2.795 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  67.3 &  4.41 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5068.765 &   2.940 &  $-$1.042 &   ... &   ... &  83.6 &  5.50 &  24.9 &  4.31 &   ... &   ... &   ... &   ... &  87.7 &  5.49 &   ... &   ... \\
   Fe\,I &  5074.748 &   4.220 &  $-$0.200 &   ... &   ... &  77.7 &  6.06 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5090.767 &   4.256 &  $-$0.400 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  23.3 &  5.34 \\
   Fe\,I &  5125.112 &   4.220 &  $-$0.140 &   ... &   ... &   ... &   ... &   ... &   ... &  39.0 &  5.34 &   ... &   ... &  61.6 &  5.66 &   ... &   ... \\
   Fe\,I &  5131.468 &   2.223 &  $-$2.515 &   ... &   ... &   ... &   ... &  17.9 &  4.72 &  50.7 &  5.57 &   ... &   ... &  61.0 &  5.63 &   ... &   ... \\
   Fe\,I &  5133.681 &   4.178 &   0.140 &   ... &   ... &   ... &   ... &  35.1 &  4.84 &  74.9 &  5.68 &   ... &   ... &  83.2 &  5.70 &   ... &   ... \\
   Fe\,I &  5141.739 &   2.424 &  $-$1.964 &  37.8 &  5.01 &  70.5 &  5.59 &   ... &   ... &  46.1 &  5.18 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5191.454 &   3.038 &  $-$0.551 &   ... &   ... &   ... &   ... &  53.5 &  4.47 &  91.3 &  5.34 &   ... &   ... &   ... &   ... &  73.1 &  4.94 \\
   Fe\,I &  5192.343 &   2.998 &  $-$0.421 &  77.2 &  4.80 &  96.6 &  5.17 &   ... &   ... &  91.1 &  5.15 &   ... &   ... &   ... &   ... &  79.1 &  4.86 \\
   Fe\,I &  5194.941 &   1.557 &  $-$2.090 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  34.0 &  4.01 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5196.059 &   4.256 &  $-$0.493 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  31.8 &  5.54 &   ... &   ... \\
   Fe\,I &  5198.711 &   2.223 &  $-$2.135 &   ... &   ... &  74.2 &  5.57 &  30.0 &  4.63 &   ... &   ... &   ... &   ... &  89.2 &  5.72 &   ... &   ... \\
   Fe\,I &  5202.335 &   2.176 &  $-$1.838 &   ... &   ... &   ... &   ... &  56.2 &  4.74 &  90.1 &  5.57 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5215.179 &   3.266 &  $-$0.871 &  63.8 &  5.34 &  86.5 &  5.75 &  21.2 &  4.44 &   ... &   ... &   ... &   ... &  81.0 &  5.57 &   ... &   ... \\
   Fe\,I &  5216.274 &   1.608 &  $-$2.150 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  49.0 &  4.35 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5217.389 &   3.211 &  $-$1.070 &  42.5 &  5.12 &  72.5 &  5.65 &  26.6 &  4.70 &  51.8 &  5.31 &   ... &   ... &  68.3 &  5.49 &   ... &   ... \\
   Fe\,I &  5227.189 &   1.557 &  $-$1.228 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  61.7 &  3.53 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5232.939 &   2.940 &  $-$0.058 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  37.8 &  3.68 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5250.645 &   2.198 &  $-$2.181 &  72.0 &  5.50 &  94.5 &  5.94 &  42.5 &  4.87 &  81.3 &  5.75 &   ... &   ... &   ... &   ... &  61.3 &  5.38 \\
   Fe\,I &  5253.461 &   3.283 &  $-$1.573 &  23.5 &  5.34 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  42.7 &  5.66 &   ... &   ... \\
   Fe\,I &  5263.305 &   3.266 &  $-$0.879 &  60.0 &  5.28 &  78.6 &  5.62 &  22.1 &  4.47 &  66.2 &  5.44 &   ... &   ... &  77.5 &  5.51 &  68.7 &  5.46 \\
   Fe\,I &  5266.555 &   2.998 &  $-$0.386 &  96.0 &  5.10 &   ... &   ... &  60.3 &  4.36 &  99.4 &  5.28 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5269.537 &   0.859 &  $-$1.321 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 140.9 &  3.91 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5270.356 &   1.608 &  $-$1.339 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  80.2 &  3.93 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5281.790 &   3.038 &  $-$0.834 &   ... &   ... &  91.0 &  5.52 &   ... &   ... &  72.5 &  5.23 &   ... &   ... &  85.1 &  5.32 &   ... &   ... \\
   Fe\,I &  5283.621 &   3.241 &  $-$0.432 &   ... &   ... &  87.2 &  5.29 &  44.3 &  4.43 &   ... &   ... &   ... &   ... &   ... &   ... &  73.5 &  5.06 \\
   Fe\,I &  5302.299 &   3.283 &  $-$0.720 &  74.2 &  5.38 &   ... &   ... &  34.4 &  4.59 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5324.178 &   3.211 &  $-$0.103 &  97.8 &  5.10 &   ... &   ... &  69.4 &  4.50 &   ... &   ... &   ... &   ... &   ... &   ... &  90.6 &  4.98 \\
   Fe\,I &  5328.038 &   0.915 &  $-$1.466 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 122.8 &  3.81 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5328.531 &   1.557 &  $-$1.850 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  44.4 &  3.92 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5339.928 &   3.266 &  $-$0.647 &  68.0 &  5.17 &   ... &   ... &  32.1 &  4.45 &  70.2 &  5.27 &   ... &   ... &   ... &   ... &  67.3 &  5.20 \\
   Fe\,I &  5364.858 &   4.445 &   0.228 &  37.5 &  5.18 &  71.5 &  5.77 &   ... &   ... &  39.1 &  5.23 &   ... &   ... &  59.6 &  5.51 &  29.2 &  5.05 \\
   Fe\,I &  5365.399 &   3.573 &  $-$1.020 &  20.6 &  5.05 &  32.5 &  5.36 &   ... &   ... &   ... &   ... &   ... &   ... &  51.0 &  5.59 &   ... &   ... \\
   Fe\,I &  5367.466 &   4.415 &   0.443 &  50.5 &  5.15 &  82.3 &  5.70 &   ... &   ... &  48.9 &  5.15 &   ... &   ... &  62.1 &  5.30 &  36.3 &  4.94 \\
   Fe\,I &  5369.958 &   4.371 &   0.536 &  51.6 &  5.02 &   ... &   ... &   ... &   ... &  63.5 &  5.27 &   ... &   ... &  76.6 &  5.40 &  47.8 &  4.99 \\
   Fe\,I &  5371.489 &   0.958 &  $-$1.645 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 100.4 &  3.70 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5383.369 &   4.312 &   0.645 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  65.7 &  5.04 &  46.4 &  4.79 \\
   Fe\,I &  5389.479 &   4.415 &  $-$0.410 &   ... &   ... &   ... &   ... &   ... &   ... &  19.8 &  5.41 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5393.167 &   3.241 &  $-$0.715 &   ... &   ... &  98.7 &  5.77 &  38.8 &  4.61 &  77.8 &  5.45 &   ... &   ... &  91.5 &  5.56 &   ... &   ... \\
   Fe\,I &  5397.127 &   0.915 &  $-$1.993 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 120.4 &  4.28 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5404.149 &   4.434 &   0.523 &  81.2 &  5.61 &   ... &   ... &  27.1 &  4.58 &  78.5 &  5.64 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5405.774 &   0.990 &  $-$1.844 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 121.4 &  4.24 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5410.910 &   4.473 &   0.398 &   ... &   ... &  67.0 &  5.55 &   ... &   ... &  54.4 &  5.36 &   ... &   ... &  59.6 &  5.37 &   ... &   ... \\
   Fe\,I &  5415.192 &   4.386 &   0.642 &  70.1 &  5.24 &   ... &   ... &   ... &   ... &  61.0 &  5.14 &   ... &   ... &  79.6 &  5.36 &   ... &   ... \\
   Fe\,I &  5424.068 &   4.320 &   0.520 &   ... &   ... &  87.0 &  5.59 &   ... &   ... &  70.0 &  5.35 &   ... &   ... &  70.6 &  5.25 &  69.3 &  5.29 \\
   Fe\,I &  5434.523 &   1.011 &  $-$2.122 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  74.1 &  3.90 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5445.042 &   4.386 &  $-$0.020 &   ... &   ... &   ... &   ... &   ... &   ... &  41.2 &  5.44 &   ... &   ... &  75.4 &  5.95 &   ... &   ... \\
   Fe\,I &  5446.916 &   0.990 &  $-$1.914 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 115.0 &  4.21 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5455.609 &   1.011 &  $-$2.091 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... & 105.0 &  4.26 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5473.900 &   4.154 &  $-$0.760 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  18.6 &  5.37 &   ... &   ... \\
   Fe\,I &  5497.516 &   1.011 &  $-$2.849 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  50.8 &  4.34 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5506.778 &   0.990 &  $-$2.797 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  50.2 &  4.25 &   ... &   ... &   ... &   ... \\
   Fe\,I &  5525.539 &   4.230 &  $-$1.084 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  17.5 &  5.74 &   ... &   ... \\
   Fe\,I &  5543.936 &   4.217 &  $-$1.140 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  17.6 &  5.79 &   ... &   ... \\
   Fe\,I &  5554.882 &   4.548 &  $-$0.440 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  23.7 &  5.64 &   ... &   ... \\
   Fe\,I &  5567.391 &   2.608 &  $-$2.564 &   ... &   ... &  41.2 &  5.91 &   ... &   ... &   ... &   ... &   ... &   ... &  19.6 &  5.35 &   ... &   ... \\
   Fe\,I &  5569.618 &   3.417 &  $-$0.486 &  57.8 &  5.01 &  89.1 &  5.56 &   ... &   ... &  60.8 &  5.10 &   ... &   ... &  98.0 &  5.64 &   ... &   ... \\
   Fe\,I &  5572.841 &   3.396 &  $-$0.275 &   ... &   ... &   ... &   ... &  43.4 &  4.43 &  93.2 &  5.48 &   ... &   ... &   ... &   ... &  62.8 &  4.89 \\
   Fe\,I &  5586.756 &   3.368 &  $-$0.120 &   ... &   ... &   ... &   ... &  56.7 &  4.46 &  90.8 &  5.24 &   ... &   ... &   ... &   ... &  75.7 &  4.91 \\
   Fe\,I &  5615.644 &   3.332 &   0.050 &  83.4 &  4.80 &   ... &   ... &  60.3 &  4.31 &  98.0 &  5.17 &   ... &   ... &   ... &   ... &  88.4 &  4.91 \\
   Fe\,I &  5624.542 &   3.417 &  $-$0.755 &  59.6 &  5.30 &  86.6 &  5.78 &  35.6 &  4.79 &  54.2 &  5.25 &   ... &   ... &  78.9 &  5.56 &  50.3 &  5.20 \\
   Fe\,I &  5658.816 &   3.396 &  $-$0.793 &  49.0 &  5.14 &   ... &   ... &  20.6 &  4.47 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5662.516 &   4.178 &  $-$0.573 &   ... &   ... &   ... &   ... &   ... &   ... &  23.4 &  5.38 &   ... &   ... &  29.8 &  5.46 &   ... &   ... \\
   Fe\,I &  5701.544 &   2.559 &  $-$2.216 &  32.6 &  5.29 &  76.2 &  6.04 &   ... &   ... &  39.9 &  5.44 &   ... &   ... &  61.5 &  5.69 &   ... &   ... \\
   Fe\,I &  5753.121 &   4.260 &  $-$0.688 &   ... &   ... &  22.7 &  5.59 &   ... &   ... &   ... &   ... &   ... &   ... &  22.3 &  5.50 &   ... &   ... \\
   Fe\,I &  5762.990 &   4.209 &  $-$0.450 &   ... &   ... &  40.8 &  5.65 &   ... &   ... &   ... &   ... &   ... &   ... &  48.0 &  5.70 &   ... &   ... \\
   Fe\,I &  5862.357 &   4.549 &  $-$0.127 &  18.1 &  5.20 &  26.5 &  5.45 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5883.813 &   3.960 &  $-$1.360 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  21.9 &  5.80 &   ... &   ... \\
   Fe\,I &  5930.173 &   4.652 &  $-$0.230 &   ... &   ... &  44.1 &  5.99 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  5934.653 &   3.928 &  $-$1.170 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  23.9 &  5.62 &   ... &   ... \\
   Fe\,I &  6003.010 &   3.881 &  $-$1.120 &   ... &   ... &  38.7 &  5.89 &   ... &   ... &   ... &   ... &   ... &   ... &  27.5 &  5.59 &   ... &   ... \\
   Fe\,I &  6024.049 &   4.548 &  $-$0.120 &   ... &   ... &  50.8 &  5.87 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  20.3 &  5.28 \\
   Fe\,I &  6055.992 &   4.733 &  $-$0.460 &  12.5 &  5.55 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  18.1 &  5.71 &   ... &   ... \\
   Fe\,I &  6065.482 &   2.608 &  $-$1.530 &   ... &   ... &  88.6 &  5.59 &  44.4 &  4.70 &  74.1 &  5.38 &   ... &   ... &   ... &   ... &  72.5 &  5.33 \\
   Fe\,I &  6137.691 &   2.588 &  $-$1.403 &  58.9 &  4.92 &  78.9 &  5.27 &   ... &   ... &  75.2 &  5.24 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6173.334 &   2.223 &  $-$2.880 &   ... &   ... &   ... &   ... &   ... &   ... &  37.6 &  5.63 &   ... &   ... &  55.0 &  5.81 &   ... &   ... \\
   Fe\,I &  6180.203 &   2.727 &  $-$2.586 &   ... &   ... &   ... &   ... &   ... &   ... &  34.5 &  5.88 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6191.558 &   2.433 &  $-$1.417 &  96.3 &  5.36 &   ... &   ... &  51.0 &  4.46 &  88.0 &  5.30 &   ... &   ... &   ... &   ... &  94.8 &  5.36 \\
   Fe\,I &  6213.429 &   2.223 &  $-$2.482 &  50.9 &  5.42 &  78.2 &  5.89 &  19.9 &  4.67 &  70.8 &  5.79 &   ... &   ... &  76.1 &  5.73 &  52.9 &  5.51 \\
   Fe\,I &  6219.279 &   2.198 &  $-$2.433 &  59.1 &  5.47 &  96.1 &  6.11 &  25.7 &  4.73 &  63.5 &  5.58 &   ... &   ... &  87.2 &  5.83 &   ... &   ... \\
   Fe\,I &  6230.722 &   2.559 &  $-$1.281 &   ... &   ... &   ... &   ... &  64.2 &  4.69 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6240.645 &   2.223 &  $-$3.233 &   ... &   ... &   ... &   ... &   ... &   ... &  14.2 &  5.43 &   ... &   ... &  33.9 &  5.82 &   ... &   ... \\
   Fe\,I &  6246.317 &   3.602 &  $-$0.733 &   ... &   ... &  67.0 &  5.61 &   ... &   ... &  37.6 &  5.12 &   ... &   ... &  50.5 &  5.27 &  32.6 &  5.06 \\
   Fe\,I &  6252.554 &   2.404 &  $-$1.687 &   ... &   ... &   ... &   ... &  58.4 &  4.81 &  96.2 &  5.69 &   ... &   ... &   ... &   ... &  78.6 &  5.32 \\
   Fe\,I &  6254.256 &   2.279 &  $-$2.443 &   ... &   ... &  64.8 &  5.72 &   ... &   ... &  62.9 &  5.68 &   ... &   ... &  66.4 &  5.62 &  54.6 &  5.57 \\
   Fe\,I &  6265.131 &   2.176 &  $-$2.550 &  40.5 &  5.27 &   ... &   ... &   ... &   ... &  58.1 &  5.58 &   ... &   ... &  76.5 &  5.75 &  37.0 &  5.27 \\
   Fe\,I &  6270.222 &   2.858 &  $-$2.464 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  36.5 &  5.87 &   ... &   ... \\
   Fe\,I &  6301.500 &   3.654 &  $-$0.718 &   ... &   ... &  61.9 &  5.58 &   ... &   ... &   ... &   ... &   ... &   ... &  49.2 &  5.29 &  32.9 &  5.11 \\
   Fe\,I &  6302.494 &   3.686 &  $-$0.973 &  26.9 &  5.24 &  42.2 &  5.57 &   ... &   ... &  28.9 &  5.29 &   ... &   ... &  31.1 &  5.27 &   ... &   ... \\
   Fe\,I &  6322.685 &   2.588 &  $-$2.426 &  14.6 &  5.06 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6335.328 &   2.198 &  $-$2.177 &  71.6 &  5.40 &   ... &   ... &  36.8 &  4.68 &  81.3 &  5.63 &   ... &   ... &  86.1 &  5.55 &   ... &   ... \\
   Fe\,I &  6336.823 &   3.686 &  $-$0.856 &   ... &   ... &  57.3 &  5.68 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  44.0 &  5.47 \\
   Fe\,I &  6344.148 &   2.433 &  $-$2.923 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  30.5 &  5.70 &   ... &   ... \\
   Fe\,I &  6393.600 &   2.433 &  $-$1.432 &  98.2 &  5.38 &   ... &   ... &  60.8 &  4.62 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6400.000 &   3.602 &  $-$0.290 &  64.7 &  5.09 &   ... &   ... &  29.5 &  4.38 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6408.018 &   3.686 &  $-$1.018 &  27.8 &  5.30 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  38.0 &  5.44 &   ... &   ... \\
   Fe\,I &  6411.647 &   3.654 &  $-$0.595 &  51.5 &  5.25 &   ... &   ... &   ... &   ... &  53.0 &  5.31 &   ... &   ... &  77.8 &  5.61 &   ... &   ... \\
   Fe\,I &  6419.942 &   4.733 &  $-$0.240 &   ... &   ... &   ... &   ... &   ... &   ... &  21.7 &  5.61 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6421.349 &   2.279 &  $-$2.027 &  78.6 &  5.46 &   ... &   ... &  44.5 &  4.76 &  95.5 &  5.85 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6430.844 &   2.176 &  $-$2.006 &  93.7 &  5.55 &   ... &   ... &  56.7 &  4.80 &   ... &   ... &   ... &   ... &   ... &   ... &  95.5 &  5.62 \\
   Fe\,I &  6481.869 &   2.279 &  $-$2.984 &   ... &   ... &  49.2 &  6.01 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6494.980 &   2.404 &  $-$1.273 &   ... &   ... &   ... &   ... &  81.4 &  4.76 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6546.238 &   2.758 &  $-$1.536 &  56.2 &  5.19 &   ... &   ... &   ... &   ... &  68.6 &  5.43 &   ... &   ... &  93.1 &  5.71 &   ... &   ... \\
   Fe\,I &  6592.913 &   2.727 &  $-$1.473 &   ... &   ... &  93.3 &  5.71 &   ... &   ... &   ... &   ... &   ... &   ... &  87.4 &  5.50 &  53.6 &  5.09 \\
   Fe\,I &  6593.870 &   2.433 &  $-$2.422 &  38.3 &  5.39 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  67.6 &  5.78 &  36.1 &  5.41 \\
   Fe\,I &  6609.110 &   2.559 &  $-$2.692 &   ... &   ... &  38.8 &  5.88 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Fe\,I &  6663.437 &   2.424 &  $-$2.479 &  48.5 &  5.60 &  66.9 &  5.93 &   ... &   ... &   ... &   ... &   ... &   ... &  60.6 &  5.71 &  38.2 &  5.49 \\
   Fe\,I &  6677.985 &   2.692 &  $-$1.418 &  84.0 &  5.42 &   ... &   ... &  41.6 &  4.60 &   ... &   ... &   ... &   ... &   ... &   ... &  86.0 &  5.49 \\
   Fe\,I &  6750.150 &   2.424 &  $-$2.621 &  27.1 &  5.36 &  48.2 &  5.79 &   ... &   ... &   ... &   ... &   ... &   ... &  40.5 &  5.54 &   ... &   ... \\
  Fe\,II &  5234.625 &   3.221 &  $-$2.180 &   ... &   ... &   ... &   ... &   ... &   ... &  70.6 &  5.47 &   ... &   ... &  74.8 &  5.49 &  74.1 &  5.43 \\
  Fe\,II &  5325.553 &   3.221 &  $-$3.160 &  20.1 &  5.44 &   ... &   ... &   ... &   ... &  19.7 &  5.44 &   ... &   ... &  31.2 &  5.70 &   ... &   ... \\
  Fe\,II &  5534.847 &   3.245 &  $-$2.750 &  32.2 &  5.32 &  56.6 &  5.72 &   ... &   ... &  41.4 &  5.52 &   ... &   ... &  64.5 &  5.89 &  32.6 &  5.31 \\
  Fe\,II &  6432.680 &   2.891 &  $-$3.570 &  26.3 &  5.57 &   ... &   ... &   ... &   ... &  27.7 &  5.61 &   ... &   ... &  37.5 &  5.79 &   ... &   ... \\
  Fe\,II &  6516.080 &   2.891 &  $-$3.310 &  42.7 &  5.61 &  60.0 &  5.87 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  44.1 &  5.62 \\
   Ni\,I &  4904.407 &   3.542 &  $-$0.170 &   ... &   ... &   ... &   ... &   ... &   ... &  28.6 &  4.10 &   ... &   ... &  43.4 &  4.32 &   ... &   ... \\
   Ni\,I &  4980.166 &   3.606 &   0.070 &   ... &   ... &   ... &   ... &   ... &   ... &  39.2 &  4.15 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ni\,I &  5017.568 &   3.539 &  $-$0.020 &   ... &   ... &  49.8 &  4.35 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ni\,I &  5035.357 &   3.635 &   0.290 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  38.7 &  3.88 &  39.5 &  3.97 \\
   Ni\,I &  5080.528 &   3.655 &   0.330 &   ... &   ... &   ... &   ... &   ... &   ... &  37.3 &  3.90 &   ... &   ... &  27.9 &  3.65 &   ... &   ... \\
   Ni\,I &  5084.089 &   3.679 &   0.030 &   ... &   ... &  58.4 &  4.59 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... \\
   Ni\,I &  5115.389 &   3.834 &  $-$0.110 &   ... &   ... &  42.8 &  4.66 &   ... &   ... &   ... &   ... &   ... &   ... &  24.7 &  4.23 &   ... &   ... \\
   Ni\,I &  5137.070 &   1.676 &  $-$1.990 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  83.1 &  4.54 &  47.6 &  4.08 \\
   Ni\,I &  5476.900 &   1.826 &  $-$0.890 &  98.9 &  3.95 &   ... &   ... &  81.1 &  3.50 &  98.3 &  4.06 &   ... &   ... &   ... &   ... &  95.8 &  3.92 \\
   Ni\,I &  5578.711 &   1.676 &  $-$2.640 &   ... &   ... &   ... &   ... &   ... &   ... &  15.9 &  4.00 &   ... &   ... &  37.4 &  4.40 &   ... &   ... \\
   Ni\,I &  5754.655 &   1.935 &  $-$2.330 &   ... &   ... &   ... &   ... &   ... &   ... &  21.7 &  4.15 &   ... &   ... &  35.7 &  4.36 &   ... &   ... \\
   Ni\,I &  6108.107 &   1.676 &  $-$2.450 &   ... &   ... &  54.5 &  4.58 &  12.2 &  3.45 &  34.8 &  4.22 &   ... &   ... &  31.1 &  4.06 &  25.0 &  4.07 \\
   Ni\,I &  6314.653 &   1.935 &  $-$1.770 &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &   ... &  25.3 &  3.56 &   ... &   ... \\
   Ni\,I &  6643.629 &   1.676 &  $-$2.300 &  38.2 &  4.07 &  55.3 &  4.40 &  12.1 &  3.26 &  51.2 &  4.31 &   ... &   ... &  67.2 &  4.45 &  44.8 &  4.25 \\
   Ni\,I &  6767.768 &   1.826 &  $-$2.170 &   ... &   ... &  82.8 &  4.86 &  14.1 &  3.38 &  42.6 &  4.21 &   ... &   ... &  51.5 &  4.26 &   ... &   ... \\
   Zn\,I &  4810.528 &   4.078 &  $-$0.137 &   ... &   ... &  74.8 &  3.13 &  25.7 &  2.06 &  45.0 &  2.64 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Y\,II &  4883.684 &   1.084 &   0.070 &   ... &   ... &   ... &   ... &  20.2 & $-$1.09 &  41.9 & $-$0.26 &   ... &   ... &   ... &   ... &   ... &   ... \\
   Y\,II &  5087.416 &   1.084 &  $-$0.170 &  25.3 & $-$0.39 &   ... &   ... &   ... &   ... &  22.1 & $-$0.45 &   ... &   ... &   ... &   ... &   ... &   ... \\
  Ba\,II &  5853.668 &   0.604 &  $-$1.000 &  47.0 & $-$0.36 &  71.4 &  0.02 &   ... &   ... &  29.7 & $-$0.66 &   ... &   ... &  37.6 & $-$0.54 &  29.6 & $-$0.66 \\
  Ba\,II &  6141.713 &   0.704 &  $-$0.076 &  92.5 & $-$0.43 & 118.4 &  0.00 &  43.8 & $-$1.62 &  89.5 & $-$0.37 &   ... &   ... &  87.4 & $-$0.55 &  86.7 & $-$0.56 \\
\enddata                                                                                                               
\end{deluxetable}                  

